On the tidal evolution of Hot Jupiters on inclined orbits

Tidal friction is thought to be important in determining the long-term spin-orbit evolution of short-period extrasolar planetary systems. Using a simple model of the orbit-averaged effects of tidal friction, we study the evolution of close-in planets on inclined orbits, due to tides. We analyse the effects of the inclusion of stellar magnetic braking by performing a phase-plane analysis of a simplified system of equations, including the braking torque. The inclusion of magnetic braking is found to be important, and its neglect can result in a very different system history. We then present the results of numerical integrations of the tidal evolution equations, where we find that it is essential to consider coupled evolution of the orbital and rotational elements, including dissipation in both the star and planet, to accurately model the evolution. The main result of our integrations is that for typical Hot Jupiters, tidal friction aligns the stellar spin with the orbit on a similar time as it causes the orbit to decay. This means that if a planet is observed to be aligned, then it probably formed coplanar. This reinforces the importance of Rossiter-McLaughlin effect observations in determining the degree of spin-orbit alignment in transiting systems. We apply these results to the XO-3 system, and constrain the tidal quality factors Q' in both the star and planet in this system. Using a model in which inertial waves are excited by tidal forcing in the outer convective envelope and dissipated by turbulent viscosity, we calculate Q' for a range of F-star models, and find it to vary considerably within this class of stars. This means that assuming a single Q' applies to all stars is probably incorrect. We propose an explanation for the survival of WASP-12 b & OGLE-TR-56 b, in terms of weak dissipation in the star.

==> ReviewersComments.tex <==

We thank the referee for a careful reading of the manuscript and 
for his helpful suggestions.  We have modified the paper as 
indicated below and as shown in bold face in the revised manuscript.
 
>> I was confused by the use of the term ?efficiency of tidal dissipation?
>> in the abstract. I had no idea what it meant until I realized that it is
>> equivalent to Q.
 
 The abstract has been updated to make this clearer.
 
>> I was pleased that on page 1, line 59, column 2, the word ?If? is used
>> regarding the initial over-packing. It is still not understood whether
>> this actually happened. However, note some evidence for such packing is
>> provided in 2 papers by Rory Barnes & me (Astrophys. J.- Letters 647,
>> L163-L166, 2006, and Astrophys. J.- Letters 665, L67-L70, 2007.
 
 This is a good point, and one of these papers has been cited in the
 introduction as evidence in favour of such close-packing.
 
>> On page 2, line 11, there should be a reference for the stated ?fact?
>> that scatterings excite inclinations. Is it a known fact? How does it
>> compare with the efficiency of exciting e?
 
 The Juric & Tremaine (2008) paper has been referred to regarding this point.
 They find that scatterings can excite the inclinations of planets with
 respect to the initial symmetry plane of the system, but that it is more
 efficient to excite eccentricity - as can be seen from Figs. 5 & 12 in
 their paper, for example.

>> On page 3, line 48, insert ?fluid? after ?homogeneous?. If the planet has
>> any rigidity, it affects k a great deal.
 
 This is a good point, and is one which we had missed. This has now been
 corrected.
 
>> On page 3, line 56, the the statement that ?Q has been found to depend in
>> a highly erratic way on the frequency? is predicated on a belief that all
>> those references actually have shown what Q values are. My opinion is
>> that no one has a clue as what the appropriate values are for Q.
>> Personally, I am very skeptical about the results in much of the
>> literature, but I am a bit out of the mainstream on that issue.
 
 All calculations of tidal dissipation (Q factors) indeed involve
 uncertainties, particularly with regards to the effective viscosity of
 turbulent convection. This makes it extremely important to treat any
 results as tentative. We have now made the statements reflect this more
 clearly.
> 
>> At the top of the second column, the authors give the usual citation to
>> Yoder and Peale for a value of Q for Jupiter. Note that result was
>> predicated on a specific scenario about the history of the Jovian system,
>> a scenario which subsequent evidence has shown cannot be possible. I
>> discussed this point in a talk at the last AAS/DPS meeting (see my
>> abstract). The Jackson et al. reference is probably more meaningful in
>> this context.
 
 Although the Yoder & Peale scenario has not been verified in detail, we
 believe the estimates of Jupiter's Q are reasonable for the purposes of our
 discussion.
 
>> In that same paragrph, the authors state that Q values must be larger for
>> WASP-12b and OGLE-TR-56b, because otherwise their life expectancies are
>> short. But why can?t their life expectancies be short? Maybe they are
>> simply the next planets to dive into their stars, as many likely have
>> before. (A new paper by Jackson et al., just submitted, emphasizes this
>> point.)
 
 It is possible for the life expectancies of these planets to be short, and
 for these planets to just be the next planets to fall into their stars.
 However, such a short inspiral time (using Q' as low as 10^5.5) would mean
 that the probability of observing such a planet would be very low (scaling
 with inspiral time / system age). Several planets with similarly short
 periods have been found, which makes it seem unlikely on probabilistic
 grounds.
 
>> Page 3, line 33, column 2:  Note spelling of achieve.
>> 
>> Not use of the expression ?stellar tide? is ambiguous. Be clear on
>> whether it is a tide raised by or raised on a star.
 
 This has been made clearer in the text.
 
>> The evolution described in Section 5.2 is (I think) the same case
>> examined in a similar way by me in Greenberg (1974, already in the
>> citation list). Perhaps a comparison of the results would be useful, just
>> to confirm whether we all got it right!
 
 Yes, the evolution considered in section 5.2 is the same as that considered
 in Greenberg (1974), though uses different dimensionless variables for the
 calculations. The results are the same, when properly compared, and we
 therefore cite this paper as a reference for the case in the absence of
 magnetic braking. Our aim is to study the inclusion of magnetic braking,
 and so we concentrate on those cases in the paper.
 
>> Page 11, line 28, column 2: For the cases considered, a very large value
>> of Q is needed to retain the observed inclination. But, alternatively,
>> couldn?t the initial value of a simply be larger?
 
 It is possible for the planet XO-3 b to start in a much wider orbit, with
 the subsequent tidal evolution of the semi-major axis occurring due to
 tidal dissipation in the star to bring the planet in towards its current
 orbit. This would require a considerably lower Q' value to explain such
 tidal migration. Such a low value of Q' is hard to explain using current
 theoretical modeling of tidal dissipation, and indeed from the calculations
 that we performed, using an appropriate stellar model, Q' ~ 10^10 or larger
 for most tidal frequencies. In addition, since the star XO-3 is an F-type
 star with similar internal structure to that of WASP-12 and OGLE-TR-56,
 this could mean a similarly lower value of Q' could apply to these systems
 as well - which we discussed above as being improbable, though is still a
 possibility.
 
>> In the rest of Section 8, I remain skeptical about whether one can
>> meaningfully determine the effective tidal Q value from this type of
>> physical modeling. Again, I am out of the mainstream on this point (but I
>> think I am correct!).
 
 The statements have been made more tentative, and it has been made clear
 that there are uncertainties in these calculations, particularly with
 regards to the effective viscosity of turbulent convection.
 



==> extrarubbish.tex <==
m_{6} &=& -1, \;\;\;\; \omega_{6} = 2n, \;\;\;\;\; \hat \omega_{6} = 2n+\Omega,
\;\;\;\;A_{6} = \frac{1}{4}\sqrt{\frac{3}{5}} \sin i\left( \cos i -1 \right), \\
m_{7} &=& -1, \;\;\;\; \omega_{7} = -2n, \;\;\;\;\; \hat \omega_{7} = -2n+\Omega,
\;\;\;\;A_{7} = \frac{1}{4}\sqrt{\frac{3}{5}} \sin i\left( \cos i +1 \right), \\
m_{11} &=& -2, \;\;\;\; \omega_{11} = 2n, \;\;\;\;\; \hat \omega_{11} = 2n+2\Omega,
\;\;\;\;A_{11} = \frac{1}{4}\sqrt{\frac{3}{20}} \left( \cos^{2} i +1
-2\cos i \right), \\
m_{12} &=& -2, \;\;\;\; \omega_{12} = -2n, \;\;\;\;\; \hat \omega_{12} = -2n+2\Omega,
\;\;\;\;A_{12} = \frac{1}{4}\sqrt{\frac{3}{20}} \left( \cos^{2} i +1
+2\cos i \right).



%NOT INCLUDED CURRENTLY!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\begin{table}%[!t]
\caption{Table of notation used throughout the paper}
\begin{center}
\begin{tabular}{llr}
  \toprule
  %\multicolumn{2}{c}{Item} \\
  %\cmidrule(r){1-2}
  Symbol & Description \\
  \midrule 
  $\mathbf{h}$   & specific orbital angular momentum vector (and its
  magnitude is $h$)\\
  $\mathbf{e}$   & eccentricity vector \\
  $\mathbf{\Omega_{1,2}}$  & spin vector of star and planet respectively
  (with corresponding magnitudes $\Omega_{1,2}$)\\
  $\mathbf{r}$ & relative separation between star and planet (with
  magnitude $r$) \\
  $a$     &  orbital semi-major axis   \\
  $n$  &  orbital mean motion ($n=\sqrt{\frac{Gm_{12}}{a^{3}}}$) \\
  $e$ & orbital eccentricity \\
  $i$ & angle of inclination between the orbital plane and the stellar equator
  (defined by $\cos^{-1}(\mathbf{\hat \Omega \cdot \hat h})$) \\
  $m_{1,2}$   & mass of star and planet respectively \\
  $m_{12}$  & total mass ($m_{1}+m_{2}$) \\
  $\mu$     & reduced mass ($\frac{m_{1}m_{2}}{m_{12}}$) \\
  $I_{1,2}$ & moment of inertia of the star and planet respectively \\
  $r_{g1}$ & dimensionless radius of gyration of star (similarly for
  planet) \\
  $\epsilon_{\star}$ & stellar mass fraction participating in tidally
  induced angular momentum exchange with the orbit \\
  $k_{1,2}$ & potential love number of order 2 for the star and planet respectively\\
  $R_{1,2}$  & radius of star and planet respectively \\
  $\alpha$ & ratio of orbital to spin angular momentum (given by
  $\frac{\mu h}{I \Omega}$) \\
  $Q^{\prime}_{1,2}$ & tidal $Q^{\prime}$-factor of star and planet respectively 
  ($Q^{\prime}_{1,2} = \frac{3Q_{1,2}}{2k_{1,2}}$), \\
  $\dot {\bmath{\omega}}_{\mathrm{mb}}$ & magnetic braking term in equation for
  $\mathbf{\dot \Omega_{1}}$ \\
  $\alpha_{\mathrm{mb}}$ & magnetic braking strength calibrated with
  observations \\
  $\gamma$ & magnetic braking correction factor, $\gamma = 1$ for G \& K
  dwarfs and $0.1$ for F-dwarfs \\
  \bottomrule
\end{tabular}
\end{center}
\end{table}

In addition, this may provide an alternative
explanation (than different disc masses) for the dip in the period
distribution of planets with
masses $>0.8 M_{J}\sin I_{\star}$ at a range of $10-100$ d around 
F-type stars, with masses larger than $1.2 M_{\odot}$ 
(\citealt{BurkertIda2007}; \citealt{Mazeh2008}), if such a dip is
statistically significant. This is because stars
of this mass or greater will contain convective cores, thus tides will
be only weakly dissipated, like for XO-3. If a planet is undergoing 
migration in a gas disc around such a star, and migrates into a 
short-period orbit, then its inward migration can be halted by its 
tidal interaction
with its host star, if the star is rotating faster than the planet's
orbital motion. If the stellar $Q^{\prime}$ is high, then the planet would have to
migrate much closer to its host star before tides could have had any
effect on the orbit. This could mean that disc torques would move the
planet closer to the star than would be necessary around a G--type star before
inward migration is halted by tidal torques - by a fractional amount $
\frac{a_{stop,G}}{a_{stop,F}} \sim
\left(\frac{Q^{\prime}_{F}}{Q^{\prime}_{G}}\right)^{2/13} \sim 4.1$ if
$Q^{\prime}_{F} = 10^{4}Q^{\prime}_{G}$ assuming the
discs around the G and F stars are the same, and that tides halt the
inward migration. Hence, there could be differences in the period distributions of
planets around G and F stars due to differences in internal structure.

\subsection{The apparent spin-synchronism of CoRoT-Exo-4b and $\tau$-Boo}

We now turn to consider the planet CoRot-Exo-4b (\citealt{Aigrain2008},
\citealt{Moutou2008}), which is a transiting $m_{2} = 0.72 M_{J}$
planet in a $P = 9.2$ d circular orbit around a late F-type star 
of mass $m_{1} = 1.16
M_{\odot}$.  The star is rotating with
a period of $P_{\star} = 8.8$ d, and similarly to $\tau$-Boo
\citep{Donati2008}, appears to be synchronised
at a mid-latitude i.e. the stellar rotation is consistent with being
synchronised plus differential rotation in the convection zone. The
age of system is estimated to be in the range $\tau_{\star} =
(0.7-2.0)$ Gyr.

Since this a late F-type star with similar properties to XO-3,
a similar tidal $Q^{\prime}\geq 10^{10}$ is
expected. Simple estimates of tidal evolution timescales (assuming $Q^{\prime}_{1} =
10^{10}$) give $\tau_{\Omega} \sim 5 \times 10^{15}$ yrs for the whole
star, which makes the tidal spin-synchronism hypothesis
implausible. Indeed, even with optimistic assumptions about the
moment of inertia of the outer convective envelope with
$\epsilon_{\star}\sim10^{-3}$, and with core-envelope decoupling assumed,
tides are not likely to be strong enough
to counteract the magnetic braking spin-down, and
$\tau_{\Omega}\gg$ the age of the universe - which we have confirmed
with numerical integrations.

On the other hand, as \cite{Aigrain2008} discuss, 
a rotation period of $9$ d is close to the peak of
the rotation period distribution for F-type stars, both during the
T-Tauri phase, and in the field. The current 
magnetic braking timescale based on simple
exponential decay is $\tau_{\mathrm{mb}} \sim 10$ Gyr (assuming weak
braking for an F--star with $\gamma=0.1$), so if the system
formed in this state, then its spin will likely not have changed
significantly since the star started on the main sequence. Depending on the initial
spin period after the dissipation of the protoplanetary disc and the
evolution of the star onto the main sequence, magnetic braking alone
may explain its current spin period. Hence, it is likely that it is
just a coincidence for this system to be in a synchronous state.

It would be interesting to see observations of the RM effect
for this system - since this would further test the outer envelope
synchronism hypothesis, as well as potentially constrain the tidal $Q^{\prime}$ of the
star. In particular, if tides have indeed synchronised the outer envelope
with the orbit, then we would also expect the orbit to have also
aligned with the spin of the star through tidal friction.

There are several other similar F--stars with close-in massive planets:
Wasp-14 \citep{Joshi2008}, $\tau$-Boo \citep{Donati2008},
XO-4 \citep{McCullough2008}, Wasp-3 \citep{Wasp32008}, HAT-P-7
\citep{HATP72008} and HD 147506 \citep{HATP22007}.

Like CoRot-Exo-4 b, $\tau$-Boo appears to
have $P\simeq P_{\star}$. $\tau$-Boo has a massive $m_{2} = 3.9
M_{J}$ planet on a $P = 3.3$ d orbit
which is synchronised with the stellar rotation at intermediate
latitudes. For this system, simple estimates of the tidal
spin-synchronisation timescale suggest that tides are
unlikely to have synchronised the whole star with the orbit \citep{Donati2008},
especially if the stellar $Q^{\prime}$ is as large as $10^{10}$. On
the other hand, if we assume only the outer envelope is spun up, and 
$\epsilon_{\star}$ is as small as $\sim10^{-3}$, then even with
$Q^{\prime} \sim 10^{10}$, $\tau_{\Omega, env}\leq \tau_{\star}$. 
It is thus possible to synchronise the outer
envelope within $\tau_{\star}$ in this simple model. But if this is
the case, since this star is very similar to XO-3,
we would return to the problem of explaining why the orbit of XO-3 b has not
aligned also. This is because we would have to reduce
$\tau_{i}$ by $\epsilon_{\star}$, since if we assume core-envelope
decoupling can occur for such stars, the outer envelope could align with the orbit
separately to the rest of the star. For XO-3, we can effectively rule
this out, unless we invoke a much higher $Q^{\prime}$ than even
$10^{10}$. 

Clearly much more work needs to be done to study the 
possibility of core-envelope
decoupling in such stars, since this has implications to the survival
and remnant inclinations of close-in planets, as well as to the
efficiency of tidal dissipation.

OGLE-TR-9 \citep{Snellen2008} is a rapidly rotating F3 star hosting a close-in massive
planetary companion. No limits on the eccentricity or spin-orbit
alignment were detected for this system. It would be especially
interesting to see RM observations, since if we observe
$i>38^{\circ}$, then the planet will be orbiting inside the
orbit-projected corotation radius. This means that the planet will be
undergoing tidally induced inspiral. If the system has high $\lambda$
and $e$, then it may have been formed by some scattering or Kozai
migration. If circular, coplanar, then some other mechanism must have
been at work to stop inward migration due to disc torques - or the
disc torques must have been weak - maybe magnetic interactions/disc
truncation/etc.??? Really want eccentricity and RM observations for
this system.

An example of
such a star is OGLE-TR-L9 \citep{Snellen2008}, which is a rapidly rotating 
F3 star hosting a close-in massive planetary companion. No limits on
the orbital eccentricity or spin-orbit alignment have been reported
for this system, but they would be especially interesting. This is
because, if tides are as weak as we predict, and no other
mechanism is more efficient at damping tides than turbulent viscosity
in the outer convection zone, then tidal dissipation in the
star will not have changed the orbit or spin properties of the
system (even though the planet will be undergoing tidal inspiral if $i
> 38^{\circ}$, since then $P > P_{\star} \cos i$). Excluding dissipation in the planet, this would mean that if
the planet has been scattered or Kozai migrated into an eccentric,
inclined orbit, then we would be able to observe the direct outcome of these
processes, enabling us to constrain these theories. On the other
hand, if the planet is found to be on a circular, aligned orbit, which
favours the gas-disc migration hypothesis, then tides are unlikely to
have been able to halt the inward migration of the planet. This might
indicate that other processes could have prevented the migration, such
as star-planet magnetic interactions \citep{Laine2008}, 
or that the gas in the disc dissipated before the planet
had migrated to the star, or that type II migration rates should be
reduced. We would very much like to encourage RM effect, 
and further radial velocity observations for this system.

An example of such a star is CoRoT-Exo-4 (\citealt{Aigrain2008},
\citealt{Moutou2008}), which hosts a transiting $m_{2} = 0.72 M_{J}$
planet in a $P = 9.2$ d circular orbit. The star is rotating with
a period of $P_{\star} = 8.8$ d, and similarly to $\tau$-Boo
\citep{Donati2008}, appears to be synchronised
at a mid-latitude i.e. the stellar rotation is consistent with being
synchronised plus differential rotation in the convection zone. The
age of system is estimated to be in the range $\tau_{\star} =
(0.7-2.0)$ Gyrs.

%AJB GREENBERG CORRECTIONS
In addition, the semi-major axis distribution
of the close-in planets does not appear to support the hypothesis that
these planets do indeed have very short inspiral times, and are just the next to
fall into their stars as many have before, since there is not a
similar distribution of planets further out
